Toward Reproducing Network Research Results Using Large Language Models

Reproducing research results in the networking community is important for both academia and industry. The current best practice typically resorts to three approaches: (1) looking for publicly available prototypes; (2) contacting the authors to get a private prototype; and (3) manually implementing a prototype following the description of the publication. However, most published network research does not have public prototypes and private prototypes are hard to get. As such, most reproducing efforts are spent on manual implementation based on the publications, which is both time and labor consuming and error-prone. In this paper, we boldly propose reproducing network research results using the emerging large language models (LLMs). In particular, we first prove its feasibility with a small-scale experiment, in which four students with essential networking knowledge each reproduces a different networking system published in prominent conferences and journals by prompt engineering ChatGPT. We report the experiment's observations and lessons and discuss future open research questions of this proposal. This work raises no ethical issue.

==> background.tex <==
\section{Background and Motivation}\label{sec:background}

\subsection{Background}

\para{A statistic of the importance of reproducing.}


\para{Why existing approaches are not enough?}


\subsection{Motivation}

\para{a brief introduction about large language models and its applications.}

\para{A small example showing code generation via prompt engineering is
feasible.}



\textbf{nlp2spec}\\
\textbf{Prompt engineering}\\
\textbf{GPT}



















==> code-java.tex <==
\definecolor{dkgreen}{rgb}{0,0.6,0}
\definecolor{gray}{rgb}{0.5,0.5,0.5}
\definecolor{mauve}{rgb}{0.58,0,0.82}
\lstdefinestyle{Java}{
    frame=tb,
    language=Java,
    aboveskip=3mm,
    belowskip=3mm,
    showstringspaces=false,
    columns=fixed,
    basicstyle={\tiny\ttfamily},
    numbers=none,
    numberstyle=\tiny\color{gray},
    keywordstyle=\color{blue},
    commentstyle=\color{dkgreen},
    stringstyle=\color{mauve},
    breaklines=true,
    breakatwhitespace=true,
    tabsize=3
}
% \documentclass{hotnets22}

% \usepackage{listings}
% \usepackage{xcolor}
% \usepackage{graphicx}




% \begin{document}

\begin{figure}[htb]

\begin{framed}

\begin{minipage}[c]{0.45\columnwidth}
\begin{lstlisting}[style=Java]
for (int i = 0; i < prefixLength; i++) {
    long bit = (prefix >> (31 - i)) & 1;
    if (bit == 1) {
        predicate = predicate.and
          (bddFactory.ithVar(i));
    } else {
        predicate = predicate.and
          (bddFactory.nithVar(i));}}
        
\end{lstlisting}
\end{minipage}
%\rule{.1pt}{36mm}
\hspace{5pt}
\begin{minipage}[c]{0.45\columnwidth}
\begin{lstlisting}[style=java]
if (r.getPriority() > rule.getPriority()) {
    int newHit = bddEngine.diff(rule.getHit(), r.getHit());
    bddEngine.deRef(rule.getHit());
    rule.setHit(newHit);
}
if (rule.getHit() == BDDEngine.BDDFalse) break;
if (r.getPriority() < rule.getPriority()) {
    int intersection = bddEngine.and(r.getHit(), rule.getHit());
    int newHit = bddEngine.diff(r.getHit(), intersection);
    bddEngine.deRef(r.getHit());
    r.setHit(newHit);

    if (intersection != BDDEngine.BDDFalse && r.getOutPort() != rule.getOutPort()) {
        changes.add(new Change(intersection, r.getOutPort(), rule.getOutPort()));
        //System.out.println("BDD:"+changes.get(0).getBdd()+" oldPort:"+changes.get(0).getOldPort().getName()+
        //        " newPort:"+changes.get(0).getNewPort().getName());
    } else {
        bddEngine.deRef(intersection);
    }
}
\end{lstlisting}
\end{minipage}

\end{framed}
\caption{Comparasion of code generated by GPT-3.5 and manually reproduced ones.}
\label{fig.java}
\end{figure}
% \end{document}


==> discussion.tex <==
\section{Discussion}\label{sec:discussion}
Some future work.

==> evaluation.tex <==
\section{Evaluation}\label{sec:eval}
Some experiment data. \cite{BGP}















==> related_work.tex <==
\section{Related Work}\label{sec:related_work}
Some previous research. What are their limitations ?

==> table1.tex <==
\begin{figure}[t] 
    \centering
\includegraphics[width=0.47\textwidth]{Figure/table1.pdf} 
    \caption{Results of normalize performance latency and relative error for the four reproduced prototypes.}
\label{fig.table}
    \end{figure}

% \begin{table}[htb]
%     \centering
%     {
%     \caption{Evaluation Results}
%     \begin{tabular}{|c|c|c|c|}
         
%         \hline  
%         \makecell[c]{Systems} & 
%         %\makecell[c]{History} &
%         \makecell[c]{Dataset} &
%         \makecell[c]{Average Relative\\ Error(\%)} &
%         \makecell[c]{Max Relative\\ Error(\%)}\\
%         \hline
%         \makecell[c]{NCFlow} &
%         %\makecell[c]{5} &
%         \makecell[c]{13} &
%         \makecell[c]{1.18} &
%         \makecell[c]{3.51}\\
%         \hline
%         \makecell[c]{Arrow} &
%         %\makecell[c]{5} &
%         \makecell[c]{2} &
%         \makecell[c]{31} &
%         \makecell[c]{32}\\
%         \hline
%         \makecell[c]{APKeep} &
%         %\makecell[c]{5} &
%         \makecell[c]{4} &
%         \makecell[c]{0} &
%         \makecell[c]{0}\\
%         \hline
%         \makecell[c]{AP} &
%         %\makecell[c]{5} &
%         \makecell[c]{3} &
%         \makecell[c]{0} &
%         \makecell[c]{0}\\
%         \hline
%     \end{tabular}
%     }

%     \label{tab:result}
% \end{table}
